A Dataset for Interactive Vision-Language Navigation with Unknown Command Feasibility

Vision-language navigation (VLN), in which an agent follows language instruction in a visual environment, has been studied under the premise that the input command is fully feasible in the environment. Yet in practice, a request may not be possible due to language ambiguity or environment changes. To study VLN with unknown command feasibility, we introduce a new dataset Mobile app Tasks with Iterative Feedback (MoTIF), where the goal is to complete a natural language command in a mobile app. Mobile apps provide a scalable domain to study real downstream uses of VLN methods. Moreover, mobile app commands provide instruction for interactive navigation, as they result in action sequences with state changes via clicking, typing, or swiping. MoTIF is the first to include feasibility annotations, containing both binary feasibility labels and fine-grained labels for why tasks are unsatisfiable. We further collect follow-up questions for ambiguous queries to enable research on task uncertainty resolution. Equipped with our dataset, we propose the new problem of feasibility prediction, in which a natural language instruction and multimodal app environment are used to predict command feasibility. MoTIF provides a more realistic app dataset as it contains many diverse environments, high-level goals, and longer action sequences than prior work. We evaluate interactive VLN methods using MoTIF, quantify the generalization ability of current approaches to new app environments, and measure the effect of task feasibility on navigation performance.

==> exps_combined.tex <==
\section{Task Feasibility}
We create a pipeline to reflect real world use of mobile app task automation in which we first reason about the input request. We train a feasibility classifier over the train split of MoTIF. After predicting feasibility on MoTIF's test set, task automation is performed for the subset of tasks predicted feasible by our classifier (see Section~\ref{sec:auto}). We describe the best performing model components below and include feature and model ablations in the Supplementary. MoTIF has 4.7k demonstrations and we reserve 10\% for testing. Note that our test set only includes (app, task) pairs for which all annotators agreed on their feasibility annotation.

\subsection{Experiments}
\label{subsec:feas}
Given the app states visited during a demonstration and its associated natural language command, the purpose of task feasibility prediction is to classify if the command can be completed or not. To determine feasibility, we expect a model needs to learn the most relevant state for the requested task and whether the functionality needed to complete it is present. Natural language reasoning about what requests result in the same task is also needed, as there are many ways to ask for the same thing, and users may request something synonymous with text present in the application (as opposed to an exact match). Our results provide an initial upper bound on performance, as input task demos can be considered the ground truth exploration needed to determine feasibility, as opposed to a learned agent's exploration.  

We propose a Multi-Layer Perceptron (MLP) baseline with two hidden layers that outputs a binary feasibility prediction. Each MLP is trained for 50 epochs with cross entropy using Stochastic Gradient Descent with a learning rate of 1e-2. The natural language command is always input to the classifier, and we ablate additional input features (app view hierarchy, app screen, or both) and how to aggregate the demonstration sequence (average, concatenation, or LSTM~\cite{lstm}). Because prior work in mobile app and website tasks has consistently neglected visual input, we intentionally investigate using language or visual only inputs to understand what features are most useful for our task. 

% All experiments include the natural language command as input, and we ablate representations of the app view hierarchy and rendered app screen to gain insight to how each modality contributes to feasibility prediction. As demonstrations are a sequence of app screens, we also experiment with different methods of aggregating demos before being passed into the MLP for the prediction. These aggregation methods include averaging (Avg), concatenating (Cat), or taking the last hidden state of an LSTM~\cite{lstm} to aggregate over the time. 
We encode the task command and view hierarchy elements per step with mean pooled features. Specifically, we try FastText~\cite{bojanowski-etal-2017-enriching} and CLIP~\cite{clip} (Visual Transformer~\cite{dosovitskiy2021image}).
% We use the trained model to obtain representations for the many view hierarchy tokens that would typically be considered out of vocabulary. 
The view hierarchy contains components such as element text (ET), IDs (ID) and class labels (CLS); we use the best combination in Table~\ref{tab:feas}, ablations are in the Supplementary. We also try Screen2Vec~\cite{screen2vec}, a semantic embedding of the view hierarchy, which represents the view hierarchy with a GUI, text, and layout embedder. 
% The GUI and text embedders make use of BERT features while the layout features are learned with an autoencoder.
To obtain visual features of the app screen, we extract ResNet152~\cite{resnet} features for the standard ten crops of each app image and CLIP representations of each app image. We also include icon features obtained from the embedding layer of a CNN trained for the downstream task of icon classification by Liu \etal~\cite{designsemantics}.

% Our best classifier C$_{feas}$ is the model trained with CLIP representations of the natural language task, view hierarchy element text and IDs, and app screen; see Table~\ref{tab:both}(c).
% \smallskip
%\noindent\textbf{Metrics.}  
For feasibility classification, we report the average F1 score over ten randomized runs, with `infeasible' as the positive class, as we care more about correctly classifying tasks that are infeasible, than misclassifying feasible tasks.
% \smallskip

% \noindent\textbf{Features.}
% We encode the natural language task and view hierarchy elements per step using mean pooled embeddings. Specifically, we try FastText~\cite{bojanowski-etal-2017-enriching} and CLIP~\cite{clip} embeddings. We use the trained model to obtain representations for the many view hierarchy tokens that would typically be considered out of vocabulary. The app view hierarchy has components such as element text (ET), IDs (ID) and class labels (CLS), which we consider separately in our experiments. We also use Screen2Vec~\cite{screen2vec}, a semantic embedding of the view hierarchy. Screen2Vec represents the view hierarchy with a GUI, text, and layout embedder; the GUI and text embedders make use of BERT features while the layout features are learned with an autoencoder. To obtain visual features, we extract ResNet152~\cite{resnet} features for the standard ten crops of each app image and CLIP representations of each app image. We also include icon features obtained from the embedding layer of a CNN trained for the downstream task of icon classification by Liu \etal~\cite{designsemantics}.

\input{res_feasibility}

\section{Task Automation}
\label{sec:auto}

Given an app and a natural language command, our goal is to interact with the app and output the sequence of commands that would complete the task.
%When training and evaluating task automation of MoTIF, we only use demos for tasks which were deemed feasible by a majority of annotators.
We provide task automation results on two versions of MoTIF to better understand its challenges.
%and transfer-only results are reported in Table~\ref{tab:automate_single} \ab{maybe the number of eval samples should be the same btw all exps in this section}.
We evaluate the test set's tasks and their full demo sequences (Table~\ref{tab:automate_full}) as well as a simplified subset, MoTIF-S, which `shortcuts' tasks to a single action (Table~\ref{tab:automate_single}). We sliced samples to the final action and manually verified which tasks were reasonable to do this with.
%MoTIF-S contains 132 samples.
%Note that task automation results for MoTIF-S and MoTIF are on the tasks predicted feasible by our classifier described in Section~\ref{subsec:feas}. 
%is done on a test split of 331 samples \ab{maybe just write 10\% of the data} and reported in Table~\ref{tab:automate_full}. 
% We experimented with augmenting MoTIF with data from RicoSCA~\cite{li-etal-2020-mapping} for training, but found this resulted in worse performance than just MoTIF alone (results in the Supplementary).

\subsection{Experiments}
% \smallskip
\noindent\textbf{Seq2Seq}~\cite{ALFRED20}
We first adapt Seq2Seq to train and evaluate MoTIF; Seq2Seq was proposed for ALFRED, a dataset for actionable natural language requests in home environments. The VLN setting is challenging as there is actual interaction with an environment at test time, and an incorrect prediction at time step $t$ will change the rest of the exploration (unlike Seq2Act which we describe next, which evaluates prediction on the ground truth sequence). Seq2Seq predicts an action class and location at each time step using the attended language task, visual features of the current state, the last predicted action, and the hidden state of an LSTM which takes the former three as input. The test-time environment and model changes are described in the Supplementary. 

% The original Seq2Seq predicts an action and binary mask at each time step. The mask represents the household object on which the action is performed. The attended language task is used as input at each time step along with visual features of the current state, the last predicted action, and the hidden state of an LSTM which takes the former three as input. We swap the deconvolutional mask prediction network for three fully connected layers that predict a point in the app screen and minimize the mean squared error.

% \textbf{Features.} As we report transfer-only results for the methods proposed by~\cite{langtoelem} and~\cite{li-etal-2020-mapping}, we defer feature description to the Supplementary. To train a modified version of Seq2Seq~\cite{ALFRED20}, we use ResNet18 features from the last convolutional layer as done in the original paper, which is needed for meaningful localization. However, we use features from five crops (four quadrants and center crop) of the original app screen as the captured app images are of much larger dimension. \ab{Need to over this implementation + seq2act}
% In addition to the features used in the original Seq2Seq model, we also include Screen2Vec representations of the state at each time step.
\smallskip
\noindent\textbf{Seq2Act}~\cite{li-etal-2020-mapping}
Seq2Act is used as a baseline to evaluate both MoTIF-S and the full sequence MoTIF test sets.
% We report the test set performance in Table~\ref{tab:automate_full} for an apples-to-apples comparison of Seq2Act to Seq2Seq, as the latter is trained and tested on MoTIF. We include Seq2Act performance on the full MoTIF dataset in the Supplementary, but its performance trends were similar to those reported on the test set.
Seq2Act approaches mobile app tasks in two stages: (action, phrase) tuple extraction and action grounding. It trains a Transformer~\cite{transformer} for each stage. The first predicts a substring, \ie, span, of the input task and an associated action.
%This means low-level instructions arethe entire pipeline depends on step by step instructions. 
The second grounds the predicted (action, phrase) tuple amongst the actionable UI elements. We describe the model and input features used in greater detail in the Supplementary.

\smallskip
\noindent\textbf{MAP}~\cite{li-etal-2020-mapping}
We also use the methods by Pasupat \etal to evaluate MoTIF-S, which were trained to map single click commands to elements on website homepages. 
The first model (MAP$_E$) embeds the command and webpage elements using Glove~\cite{pennington2014glove}. The second model (MAP$_A$) builds an alignment matrix between the input command and web elements via multiple convolutions and max pooling. In both, a linear scoring function learns to maximize the log likelihood of the correct website element given the concatenated embeddings. Model variants with $N$ (\eg, MAP$_{EN}$) refer to neighbor web elements being included as additional input. 

% Lastly, we use Seq2Seq~\cite{ALFRED20} to train and evaluate MoTIF. The Seq2Seq model was proposed as a VLN model for the ALFRED dataset, which contains actionable natural language requests for tasks in household environments. A key difference from Seq2Act is the VLN setting: there is actual interaction with an environment at test time, and an incorrect prediction at time step $t$ will change the rest of the exploration (unlike Seq2Act which evaluates prediction on the ground truth exploration sequence). A description of MoTIF's test-time environment is provided in the Supplementary.

% The original Seq2Seq predicts an action and binary mask at each time step. The mask represents the household object on which the action is performed. The attended language task is used as input at each time step along with visual features of the current state, the last predicted action, and the hidden state of an LSTM which takes the former three as input. We swap the deconvolutional mask prediction network for three fully connected layers that predict a point in the app screen and minimize the mean squared error.

% \textbf{Features.} As we report transfer-only results for the methods proposed by~\cite{langtoelem} and~\cite{li-etal-2020-mapping}, we defer feature description to the Supplementary. To train a modified version of Seq2Seq~\cite{ALFRED20}, we use ResNet18 features from the last convolutional layer as done in the original paper, which is needed for meaningful localization. However, we use features from five crops (four quadrants and center crop) of the original app screen as the captured app images are of much larger dimension. \ab{Need to over this implementation + seq2act}
% In addition to the features used in the original Seq2Seq model, we also include Screen2Vec representations of the state at each time step.

\smallskip
\noindent\textbf{Metrics}
We report accuracy for MoTIF-S, which is classification accuracy over the UI elements. Table~\ref{tab:automate_single} also compares when the full, original task language was input vs. the shortcut version which slices the  language to the final task. \Eg, for the original task `Go to lullabies and select Chants of Tibet' requested in a sleep cycle app, we can input this full instruction or shortcut it to `select Chants of Tibet' which only requires reasoning at the current time step. 

When evaluating the full sequence MoTIF, complete and partial accuracy are reported per~\cite{li-etal-2020-mapping}: the complete score is 1 if two sequences have the same length and the same prediction at each step, else 0. The partial score is the fraction of predicted steps that match the ground-truth sequence. We report complete and partial accuracy for action prediction (Action), action grounding (Ground), or both action and grounding jointly. 

\input{res_auto}

==> introduction_2.tex <==
\section{Introduction}

\begin{figure}[t]
\centering
    \includegraphics[scale=0.0425]{3motivation_motif.drawio.png}
    \label{fig:motivation}
        \caption{Example MoTIF tasks. Task inputs are free form natural language commands which may not be possible in the app environment. At each time step, a task demonstration consists of action coordinates (\ie, where clicking, typing, or scrolling occurs) and the app screen and view hierarchy (illustrated behind it). We also illustrate the captured app modalities: the rendered screen and the app view hierarchy, which contains metadata about all elements such as their Android class, resource ID, and text}
\end{figure}

\begin{table*}[ht]
\setlength{\tabcolsep}{2.2575pt}
%   \renewcommand\arraystretch{0.95}
    \centering
        \caption{Comparison of MoTIF to existing datasets. For language comparison, we consider the number of natural language commands, command granularity, and existence of feasibility annotations. For visual comparison, we consider the number of environments and views (we report the median number of views, \ie, the number of visited states during a demonstration), if the rendered screen is captured (\ie, app or website screenshot), and the actions it contains (click $_{ \includegraphics[scale=0.05]{click-tight.png}}$, swipe$_{\includegraphics[scale=0.085]{swipe_2.jpg}}$, or type $_{ \includegraphics[scale=0.04]{keyboard.jpg}}$)}
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
    \hline
       \multirow{2}{*}{Dataset} & \multicolumn{3}{c|}{Language Annotations} & \multicolumn{4}{c|}{Digital Dataset Environment} \\ 
    \cline{2-8}
         & \# NL & Task & \multirow{2}{*}{Feas.} & \# & \multirow{2}{*}{Screen} & \# & Actions  \\
                  & tasks & granularity & & envs. & & views & included \\
         \hline
        % \textbf{(a) House} & & & & & & &  \\
        % R2R~\cite{Anderson_2018_CVPR_NAV} & & & & & & & \\
         %& 21,567 & Low & \color{red}{\ding{55}} & 90 &  \color{green}{\ding{51}}  & -- & -- & \color{green}{\ding{51}}\\
        %  \hspace{4mm} EQA~\cite{embodiedqa} & 0 & High & \color{red}{\ding{55}} & 45,000 & \color{red}{\ding{55}} & -- & --  &  \color{green}{\ding{51}} \\
        %  IQA~\cite{IQA} & & & & & & & \\
         % & 30 & 0 & -- &  & & \color{green}{\ding{51}} & \color{red}{\ding{55}} & \color{red}{\ding{55}}\\
        %  ALFRED~\cite{ALFRED20} & & & & & & & \\
         % 25,743 & High + Low &  \color{red}{\ding{55}} & 120 &\color{red}{\ding{55}} & -- & --  &  \color{green}{\ding{51}}\\
        %  \hline
       
          \textbf{(a) Webpage} & & & & & & & \\
        MiniWoB~\cite{wob} &  0  & High & \color{red}{\ding{55}} & 100  & \color{red}{\ding{55}}& 1 & \multirow{2}{*}{\includegraphics[scale=0.06]{click-tight.png}} \\
        Pasupat~\etal~\cite{langtoelem} & 50,000 & Low & \color{red}{\ding{55}} & 1,800 & \color{red}{\ding{55}} &  1 & \\
         \hline
         \textbf{(b) Mobile App} & & & & & & & \\ 
         Rico~\cite{rico} & 0 & N/A & \color{red}{\ding{55}} & 9,700 & \color{green}{\ding{51}}& 6.7 & --\\
         PIXELHELP~\cite{li-etal-2020-mapping} & 187 &  Low & \color{red}{\ding{55}} & 4 &\color{red}{\ding{55}}& 4  &\includegraphics[scale=0.06]{click-tight.png} \\
         MoTIF (Ours) & 6,100 & High,Low & \color{green}{\ding{51}} & 125  & \color{green}{\ding{51}} & 8 &  \includegraphics[scale=0.06]{click-tight.png} \includegraphics[scale=0.095]{swipe_2.jpg}\includegraphics[scale=0.045]{keyboard.jpg} \\
         \hline
    \end{tabular}
    \label{tab:compare}
\end{table*}

Websites and mobile apps provide rich multimodal data for research in web and app task automation~\cite{navigateweb,domqnet,li-etal-2020-mapping,wge,langtoelem,wob}, app design~\cite{rico,erica,designsemantics}, and human-computer interfaces~\cite{sugilite,convobreak,demoplusLi2021}, as well as related vision-language tasks such as document understanding~\cite{appalaraju2021docformer,Li_2021_CVPR,canvasvae}, vision-language navigation~\cite{Anderson_2018_CVPR_NAV,embodiedqa,IQA}, and task relevance prediction~\cite{Gardner2020DeterminingQP,vizwiz,ray2016question}. The mobile app domain not only provides interesting data for academic research purposes, but also for high impact use in downstream applications. For example, with improved app understanding and app navigation models, app layouts or visual features can be made more intuitive and accessible. Another significant downstream use-case includes automating natural language queries in apps, to assist people who are not able to complete the task themselves, either situationally (\eg, while driving) or physically (\eg, users who are low-vision or blind). Improving mobile app task automation methods for natural language requests could better balance the capabilities of current assistive technologies, which typically lack agency or flexibility~\cite{screenreader}: screen readers are primarily used for web browsing and information consumption (lacking agency), while interactive tools like virtual assistants (\eg, Siri, Alexa) have limited, structured commands (lacking flexibility). 

Despite the significant opportunity for positive societal impact with mobile app data, the data used in prior work has failed to capture the realism needed to do so. First, existing mobile app task automation methods train only on synthetic language data, created using well defined templates such as ``click on \textbf{x},'' where x is automatically generated. Additionally, the training paradigm used for the state of the art mobile app task automation assumes step-by-step instruction~\cite{li-etal-2020-mapping}. Not only does this set up avoid the challenges that arise with natural language like ambiguous instruction, but it also does not reflect downstream use, where users would ask for the high level goal as opposed to providing step-by-step instruction. 

When high level natural language goals are requested, the request may not be feasible in the provided app. This could occur for various reasons: the request may be ambiguous, state dependent, refer to functionality no longer available, or be possible in another app but not the current app. Task feasibility has been studied in other contexts such as question relevance for text-only~\cite{Gardner2020DeterminingQP} and visual question answering~\cite{vizwiz,ray2016question},
%, where for the latter inputs are single image-text pairs, 
but never for interactive multimodal data like mobile app action sequences.
%, they have focused on the extreme case of language being completely unrelated to the visual input it is paired with. 
%However, these cases have 

%do not include natural language ambiguity or infeasibility that arises due to lack of familiarity with a new environment. 
%VizWiz~\cite{vizwiz} introduced a visual question answering dataset for images taken by people that are blind, resulting in questions which may not be answerable from the captured image. However, 87\% of the unanswerable train samples had at least one annotator which deemed it unanswerable due to distinct visual failures like image blur or flash. These works have been necessary to study particular or more obvious cases of infeasible language requests. However, they do not include natural language ambiguity or infeasibility that arises due to lack of familiarity with a new environment. 
% Additionally, images that cannot be used to answer visual questions are easily classified as such, as they often contain blurred or random scenes (\eg, the floor). 
%Gardner \etal~\cite{Gardner2020DeterminingQP} explored question-answer plausibility prediction, but the questions used were generated from a bot, which could result in extraneous questions that are easy to classify as implausible. \

In addition to lacking language instruction realism, prior work for app task automation only evaluates tasks for app environments that were seen during training. Generalization to unseen apps and unseen tasks is an important issue for the mobile app domain, as the growing number of existing mobile apps makes it impossible to collect data for every possible app. Furthermore, benchmarking on unseen apps versus unseen tasks versus both will provide insight to which part of the problem is more difficult for models to solve (\eg, do we need more generic app representations? do we need better attention mechanisms between apps and the input language instruction?).

To study these challenges, we propose Mobile app Tasks with Iterative Feedback (MoTIF)\footnote{Code and data will be released upon acceptance for anonymity purposes}, the largest dataset designed to support interactive methods for completing natural language tasks in mobile apps. MoTIF provides greater linguistic complexity for interactive tasks with over 6.1k free form natural language commands across 125 Android apps. We have collected 4.7k task demonstration samples for apps across fifteen Android categories thus far. A sample includes the natural language command (\ie, task), app view hierarchy, app screen, and action coordinates for each time step, as shown in Figure~\ref{fig:motivation}. MoTIF uniquely includes binary feasibility annotations for each task, subclass annotations for why tasks are infeasible, and natural language follow up questions (see Figure~\ref{fig:infeas_motif}). 

We show additional differences between MoTIF and existing datasets in Table~\ref{tab:compare}. Prior work in automating web tasks~\cite{langtoelem,wob} limit user interaction to one screen,
unlike MoTIF, which has task demos with a median of 8 visited screens (\# views in Table~\ref{tab:compare}). PIXELHELP~\cite{li-etal-2020-mapping} was recently introduced as a small mobile app dataset, but most commands are device specific. \Ie, the tasks refer to the phone itself, such as `in the top control menu click the battery saver,' and are not in-app tasks like those in Figure~\ref{fig:motivation}. This is a key distinction, as PIXELHELP closely mimics existing virtual assistant abilities. MoTIF also contains clicking, typing and swiping actions, whereas PIXELHELP only contains clicking.

%We present results for the portion of MoTIF collected thus far\footnote{Code and data will be released upon acceptance for anonymity purposes}, which is sufficient to understand pitfalls of prior work.
% In addition to the dearth of research on more nuanced task feasibility, all prior work studies static image-text pairs, and not interactive visual environments where an AI agent may require navigation and state change to complete a request. Vision language navigation (VLN) datasets and models have not tackled such problems, and often require step-by-step user instruction (\ie, low task granularity) \cite{Anderson_2018_CVPR_NAV,ALFRED20}.

% MoTIF will allow for new research toward predicting task ambiguity that would arise in real use cases of these AI systems. Our infeasible tasks are always relevant to the Android app category they are paired with, making them challenging due to their inherent relevance to the visual environment. 
We propose a baseline model for task feasibility prediction and confirm app exploration is necessary. Surprisingly, we find that prior representation learning approaches specific to the mobile app domain do not result in the best performance for our feasibility classifier. 
We then evaluate three methods for automating MoTIF's app tasks and examine performance failures using our generalization splits. We find ... Tease out results ...

% MoTIF will also allow for new research toward predicting task ambiguity that would arise in real use cases of these AI systems. Our infeasible tasks are always relevant to the Android app category they are paired with, making them challenging due to their inherent relevance to the visual environment. We propose a baseline model for task feasibility prediction and confirm exploration is necessary, which is notably different from prior work like VizWiz~\cite{vizwiz}. Surprisingly, we find that prior representation learning approaches specific to the mobile app domain do not result in the best performance for our feasibility classifier. We also evaluate off the shelf and trained from scratch models for automating MoTIF's app tasks and examine performance failures.

% We also collect demos of the same task across multiple apps to encourage research in task generalization, so that resulting tools are robust to domain shift and ultimately higher impact in application.

%We acknowledge MoTIF is not on the scale of huge pretraining datasets used for other vision-language tasks (\eg, Alt-Text~\cite{jia2021scaling}, JFT-300M~\cite{jft300}), as it is very expensive and time consuming to collect. MoTIF is nonetheless useful to the research community as it is extremely realistic and can be used to evaluate how existing  methods actually solve language-based digital tasks.

We summarize our contributions below:
\begin{itemize}
% \setlength\itemsep{0em}
    \item A new dataset, Mobile app Tasks with Iterative Feedback (MoTIF), with free form natural language commands for interactive goals in mobile apps. It has natural language tasks for the most visual environments to date and is the only to include the app screen in its annotations. MoTIF uniquely has multiple types of interactions including clicking, swiping and typing actions, and a subset of infeasible tasks.
    \item A new vision-language task: mobile app task feasibility classification, along with subclass annotations on why tasks are infeasible and follow up questions for research toward resolving task uncertainty via dialogue. 
    \item Benchmarks for feasibility classification and task automation with MoTIF. A thorough feature exploration is performed for feasibility classification to understand the role of vision and language in understanding task feasibility. We compare several methods on mobile app task automation using different test splits: seen apps with unseen tasks, unseen apps with seen tasks, and unseen apps with unseen tasks. We provide generalization analysis as well as qualitative discussion of failures, providing insights for future work.
\end{itemize}


==> res_auto.tex <==
\subsection{Results}
\label{autoperf}
\begin{table}[t]
    \centering
        \caption{Mobile app task automation on MoTIF. We evaluate the Seq2Seq navigation model trained from scratch and the double transformer grounding model Seq2Act off the shelf}
    \begin{tabular}{|l|c|c|c|c|}
    \hline
      Model & Action & Ground & Action + Ground \\ 
        \hline
        \textbf{Seq2Seq}~\cite{ALFRED20} & & & \\
  
  \hspace{1mm} Complete & 22.3 & 0.6 & 0.6  \\ % 12.5 & 0.3 & 0.3\\ 
 \hspace{1mm} Partial & \underline{66.6} & 3.7 & 3.7 \\ % 68.0 & 1.6 & 1.5 \\
        \hline
        \textbf{Seq2Act}~\cite{li-etal-2020-mapping} & & & \\
        \hspace{1mm} Complete & \underline{56.5} & \underline{30.1} & \underline{20.2} \\ % 44.6 & 26.2 & 17.5 \\ 
        \hspace{1mm} Partial & 59.6 & \underline{34.5} & \underline{24.6} \\ % 49.3 & 29.9 & 21.3\\ 
        \hline
    \end{tabular}
    \label{tab:automate_full}
    \vspace{-3mm}
\end{table}

%  We now analyze the results for task automation on MoTIF-S (Table~\ref{tab:automate_single}) and MoTIF (Table~\ref{tab:automate_full}). 
\begin{table}[b]
    \centering
        \caption{Mobile app task completion on MoTIF-S. We evaluate the MAP embedding and alignment models, with or without neighbor elements as input and the double transformer model Seq2Act}
    \begin{tabular}{|l|c|c|}
    \hline
      Method & Full & Shortcut \\
       \hline
     \textbf{Random} & \multicolumn{2}{c|}{3.5}\\
      \hline 
     \textbf{MAP}~\cite{langtoelem} & &\\
      \hspace{1mm} MAP$_E$ & 17.4 & 22.0 \\
      \hspace{1mm} MAP$_{EN}$ & 21.1 & 21.1 \\
     \hspace{1mm} MAP$_{A}$ & 26.5 & 28.0 \\
     \hspace{1mm} MAP$_{AN}$ & 25.8 & 31.1 \\
      \hline
      \textbf{Seq2Act}~\cite{li-etal-2020-mapping} &\underline{35.6} & \underline{69.7}\\
    %  \hspace{1mm}  Seq2Act & 19.6\% & 26.6\% \\
      \hline
    \end{tabular}
    \label{tab:automate_single}
\end{table}

% We report task completion performance on MoTIF in Table~\ref{tab:automate_full} by evaluating action prediction, grounding prediction, and both action + grounding prediction results. The complete action + grounding results are equivalent to the percentage of tasks that were solved. 

% The complete pipeline with Seq2Act reflects low performance, with only 17.5\% of tasks completely solved. 

% We can compare performance when evaluating action predict only versus ground prediction, or both. 
Seq2Act achieves the highest performance for all metrics except partial sequence action prediction (Table~\ref{tab:automate_full} Seq2Seq achieves 66.6\% accuracy compared to 59.6\% of Seq2Act). Seq2Seq is trained from scratch on MoTIF and performs the much more challenging task of screen localization, where a point in the app screen is predicted at each time step, unlike Seq2Act which predicts over the leaf UI elements. The VLN setup also requires environment interaction and may not recover from a wrong prediction. As Seq2Seq has lower results, we defer its discussion to the Supplementary.  

Comparing the columns of Table~\ref{tab:automate_full}, Seq2Act's action prediction is much better than its grounding, which is sensible as it only predicts actions over four classes (click, type, swipe, and EOS), much fewer than 28, the average number of leaf UI objects grounded over in MoTIF-S. Compounding errors result in the lowest accuracy when evaluating Action + Ground. Seq2Act was originally evaluated with PIXELHELP~\cite{li-etal-2020-mapping} and achieved 70.6\% complete Action + Ground accuracy. It is clear PIXELHELP's click-only Gmail, Google Photos, Google Chrome, and device tasks do not reflect the model's ability on a greater variety of apps or tasks, nor on swiping or typing actions. 
%\ab{make sure the MoTIF test set also includes typing and or swiping, or else this statement isn't a valid point}. 

We look to further understand what makes MoTIF challenging for Seq2Act with MoTIF-S. 
%Results are provided when the full original task is used as input as well as the single shortcut subtask (full versus shortcut columns in Table~\ref{tab:automate_single}). 
%%%%%%%%%%%%%%%%%%%
While performance is significantly higher, the results in Table~\ref{tab:automate_single} demonstrate that MoTIF's natural language task inputs and mobile app environments are difficult even when simplified to single-action tasks.
The MAP models' transfer performance is notably lower than Seq2Act due to domain shift from websites, unlike Seq2Act which was trained on mobile app data. However, we can still gain insight from MAP results: including spatial context via neighboring elements only helps in some cases (\eg, Table~\ref{tab:automate_single} MAP$_{EN}$ 21.1\% vs. MAP$_{E}$ 17.4\% Full). This provides more evidence that hierarchical vision-language features may help learn context and better capture neighboring elements, as these text-only features fall short. 

\begin{figure}
    \centering
    \includegraphics[scale=0.03725]{qual_s2a.drawio.png}
    \caption{\small Examples of Seq2Act text matching. Green boxes are valid predictions, red are invalid predictions, and black are ground truth valid UI elements for the task input. On the left we see a valid prediction that matches the task text for `notification' directly to the UI in the app Pinterest. On the right we see a failure case of Seq2Act overly relying on text matching, as it matches `my' in the input task to the UI element `My favorite' in the Opera news app}
    \label{fig:qual}
\end{figure}

Looking at misclassifications, we find one culprit to be Seq2Act overly relying on matching input task text to view hierarchy text. In Figure~\ref{fig:qual}, we show Seq2Act's text matching tendency, which can result in failure. For example, Seq2Act predicts the UI element with the word `my' in it for the input command `go to my profile.' These results, in addition to the high visual performance from the feasibility classifier, verifies the need for visual input to correct model bias to match input task text directly to the view hierarchy.  

Both methods perform worse when the natural language input is not sliced to the substring of the final action. 
%This is more expected for MAP, which was trained and evaluated on single action tasks. 
% Seq2Act was trained on multitask sequences and its first transformer learned to map an input language task to an (action, phrase) pair, where the phrase is a substring of the original task. 
Thus, most of the poor performance originates from the (action, phrase) tuple extraction model, which cannot reason about the current state the demonstration has been `shortcut' to. Seq2Act relies on a one-to-one correspondence of the task input to the action sequence, which is again, extremely unlikely in application. Ideally, a vision-language model should recognize what portion of a task has already been completed. In future work, it may be useful to add explicit losses to  predict how much of a task has been completed given the current observed state, or predicting whether we are `before' or `after' a particular subtask of our final goal.
%Learning the number of subtasks a particular input request has may be a helpful tool to generalize the current Seq2Act paradigm.
%many steps have been completed/how far we are from final target}

% We find the alignment model outperforms the embedding model, unlike the results reported by Pasupat \etal for their website task. This may be a result of the single-action MoTIF-S tasks mostly being a string matching problem, for which they report the alignment model to be over twice as effective.

% Seq2Act largely outperforms MAP variants with over twice the accuracy on MoTIF-S, but its accuracy is still low given that it was trained on Android apps and multitask sequences. Seq2Act was evaluated with PIXELHELP~\cite{li-etal-2020-mapping}, a small set of click-only tasks that only cover Gmail, Google Photos, Google Chrome, and Android device commands. Seq2Act performs very well on this test set, but no performance is reported on a greater variety of apps or language inputs, nor on swiping or typing action.s \ab{make sure the MoTIF test set also includes typing and or swiping, or else this statement isn't a valid point}. 

Seq2Act was also trained on sequences which were automatically generated and built to have separating clauses or punctuation. This domain shift may cause the model to fail to recognize that the entire input string should be predicted as the task substring, and then the incorrect (action, phrase) leads to grounding failure. This assumption is particularly bad when we consider that systems for automating mobile app tasks would likely have spoken interfaces, where such punctuation is not available.
% \ab{actually look at 10 randomly sampled span predictions}.

\section{Task Automation with Feasibility}
We now discuss the performance achieved with the best combined pipeline (Table~\ref{tab:both}) and next steps given the failures of our baselines for MoTIF's new problem of task feasibility prediction as well as mobile app task automation.
%For the joint performance, we look to see how much can be attributed to the feasibility classifier. I
% In Table~\ref{tab:classifier}, 
A total of 8.6\% of test samples were incorrectly predicted as feasible and have zero accuracy in the task automation portion of our pipeline.
% We include the prediction confusion matrix for our best feasibility classifier in the Supplementary. 
If we only consider the samples correctly predicted as feasible, complete Action + Ground performance would be nearly 4\% higher (20.2\% in Table~\ref{tab:automate_full} vs. 16.8\% in Table~\ref{tab:both}). Most of the poor complete pipeline performance originates from the task completion failures.
 
% \begin{table}[t]
%     \centering
%     \begin{tabular}{l|c|c}
    
%      & GT Feasible &  GT Infeasible \\
%     \hline
%      Predicted Feasible & 347 & 39 \\
%      Predicted Infeasible & 18 & 50 \\
%     \end{tabular}
%     \caption{Feasibility classifier predictions on the MoTIF test set.}
%     \label{tab:classifier}
% \end{table}

\begin{table}[t]
    \centering
        \caption{Task completion on MoTIF with the full pipeline. The subset of tasks predicted as feasible are input to Seq2Act~\cite{li-etal-2020-mapping}}
    \setlength{\tabcolsep}{4.3pt}
    \begin{tabular}{|l|c|c|c|c|}
    \hline
      Complete Pipeline & Action & Ground & Action + Ground \\ 
%         \hline
%         \textbf{C$_{feas}$ + Seq2Seq} & & & \\
  
%   \hspace{1mm} Complete & & & \\ 
%  \hspace{1mm} Partial & & & \\
        \hline
        \textbf{C$_{feas}$ + Seq2Act} & & & \\
        \hspace{1mm} Complete & 47.0 & 25.0 & 16.8\\ % 39.8 & 23.4 & 15.7 \\ 
        \hspace{1mm} Partial & 49.6 & 28.7 & 20.5 \\ % 44.0 & 26.7 & 19.0 \\ 
        \hline
    \end{tabular}
    \label{tab:both}
        % \vspace{-2mm}
\end{table}

% The low results on task feasibility prediction and task automation show that MoTIF does indeed create a more realistic setting, and motivates new research to bridge the gap with human ability on such tasks. Our experiments show potential next steps: %where there is room for improvement:
Still, task feasibility classification results are low at only a maximal 61.1 F1 score, given that the input demos serve as the oracle exploration needed to determine feasibility; adapting the training paradigm to use learned explorations is a necessary next step. Our classifier ablations demonstrate that visual inputs are useful for feasibility prediction, and research toward better mobile app features that actually use the rendered screen could provide performance boosts. Similarly for task automation, neighboring UI elements did not provide significant context with MAP to help classify the correct UI element for a MoTIF-S task. Building hierarchical visual and textual features may provide stronger context clues. We also hope to perform experiments classifying why tasks are not feasible and automating question generation in response, making use of MoTIF's subclass annotations for infeasible tasks and follow up questions.

In addition to needing improved representations, models for completing mobile app tasks should be able to recognize when subtasks have been completed, and current methods only succeed with step-by-step instruction. A necessary next step is to better model the current state and map high level goals to subtasks. Adding auxiliary tasks like predicting if a subtask has been reached given the current state may help build higher level reasoning about task completion instead of only modeling tasks in a Markovian world. 

We lastly discuss the ethical impact this work may have. The collection of MoTIF was designed to ensure no personally identifiable information is captured. But, in downstream use of mobile app task automation, user privacy and security is a concern. People who use assistive technology (\eg, people who are blind) already expose sensitive information to other humans to receive help~\cite{Akter2020IAU,visprivacy}. To mitigate potential harm from automating app tasks, deployment of our research can be limited to apps which do not require log in information; these apps are less likely to include name, address, or payment data. MoTIF does not have tasks which require payment, and we can blacklist payment related tasks to prevent fraud and other undesired outcomes. We also acknowledge that improving task feasibility prediction can have more distant negative outcomes, as improved vision-language reasoning could be used for surveillance.

==> res_feasibility.tex <==
\subsection{Results}
% We first report the task feasibility and task completion results separately. In Section \ref{feasperf}, we review the primary feature study for our feasibility classifier and discuss directions for improving feasibility reasoning. Next, we analyze the task completion performance and unique challenges revealed by MoTIF in Section~\ref{autoperf}. We evaluate our baseline under the standard MoTIF test set as well as a simplified version for additional insight.
\begin{table}[t]
% \renewcommand{\arraystretch}{1.05}
% \setlength{\tabcolsep}{3.69pt}
    \centering
        \caption{Task feasibility F1 score using our MLP. We ablate input features and how demo sequences are aggregated. The random baseline predicts a feasibility label given the train set distribution}
    \begin{tabular}{|l|c|c|c|}
    \hline
       \multirow{2}{*}{\textbf{C}$_{feas}$ Input Features} & \multicolumn{3}{c|}{Demo Aggregation}\\
       \cline{2-4}
       & Avg & Cat & LSTM \\ %& Mean \\
       \hline
       \textbf{Random} & \multicolumn{3}{c|}{20.1}\\
       \hline
     \textbf{(a) View Hierarchy} & & & \\ %& \\
    %  FastText (ET + ID) & & & & \\
    % \hspace{4mm} ET & 22.8 & 44.3 & 37.0 & 34.7
    %  \\
     FastText (ET + ID) & 16.7 & 43.6 & 34.1 \\ %& 31.5
     
    % \hspace{4mm} ET + ID + CLS & 19.7 & 39.6 & 36.2 & 31.8 \\
    % CLIP & & & & \\
    % \hspace{4mm} ET & 27.0 & 48.4 & 35.9 & 37.1
    %  \\
     CLIP (ET + ID) & 28.0 & 50.9 & 36.2 %& 38.4
     \\
    % \hspace{4mm} ET + ID + CLS & 29.6 & 49.2 & 35.2 & 38.0 \\
      Screen2Vec & 25.9 & 33.7 & 36.0 \\ %& 31.9 \\
      \hline
      \textbf{(b) App Screen} & & & \\ % & \\
       ResNet & 31.3 & 41.9 & 35.9 \\ %& 36.4 \\
     Icons & 0.4 & 40.0 & 15.2 \\% & 18.5 \\
     CLIP & 44.7 & 58.2 & \underline{42.8} \\% & 48.6 \\
      \hline
      \textbf{(c) Best Combination} & & & \\% & \\
      CLIP (Screen + ET + ID) & \underline{44.8} & \underline{61.1} & 40.9 \\ %& \textbf{48.9}\\
      \hline
    %   \multicolumn{4}{c}{}\\
    % \hline 
    %   Complete Pipeline & Act & Ground & Act + Ground \\ 
%         \hline
%         \textbf{C$_{feas}$ + Seq2Seq} & & & \\
  
%   \hspace{1mm} Complete & & & \\ 
%  \hspace{1mm} Partial & & & \\
        % \hline
        % \textbf{C$_{feas}$ + Seq2Act} & & & \\
        % \hspace{1mm} Complete & 39.8 & 23.4 & 15.7 \\ 
        % \hspace{1mm} Partial & 44.0 & 26.7 & 19.0 \\ 
        % \hline
    \end{tabular}
    \label{tab:feas}
\end{table} 
% \subsection{Task Feasibility}
\label{feasperf}
Our best task feasibility classifier (Table~\ref{tab:feas}(c)) achieves an F1 score of 61.1 when CLIP embeds the task, view hierarchy, and app screen. This is still fairly low, and feature ablations demonstrate room to improve both the language and visual representations. While CLIP has shown significant performance gains in other vision-language tasks, it is somewhat surprising that domain-specific embeddings (\eg, Screen2Vec) are not as competitive. The combination of view hierarchy and app screen features does not largely outperform the app screen CLIP results (and does worse with LSTM aggregation), suggesting a need for a better vision-language encoding which can pull features together from different modalities such as the view hierarchy.

Table~\ref{tab:feas}(a) compares methods of encoding the view hierarchy. Using CLIP for view hierarchy elements results in notably better performance than FastText, albeit less significant when input demos are aggregated with an LSTM. Our final view hierarchy embedding comes from Screen2Vec. Despite being trained on mobile app data, it performs worse than CLIP and on par with FastText. Screen2Vec may not capture enough low level view hierarchy information to predict feasibility, and methods trained on huge data, even if from another domain, are more powerful.

In Table~\ref{tab:feas}(b) we ablate over visual features of the app screen.
While icon representations are trained on images from the same domain as MoTIF, they are significantly less effective than ResNet and CLIP. The F1 score nearly drops to zero when the average icon feature is used, illustrating that the average icon does not carry useful information for feasibility classification. Icon features may be too low-level or require improved aggregation methods.
%While both ResNet and CLIP were trained on natural images, CLIP is able to have high gains compared to ResNet, illustrating the utility of contrastive learning. 

When comparing demonstration aggregation methods (averaging vs. concatenating vs. LSTM), there is a trend that concatenating time steps is the best method, suggesting a sequential representation of demonstration time steps is needed.
However, when the best representations for the view hierarchy and app screen are combined in Table~\ref{tab:feas}(c), averaging manages to outperform the LSTM performance. 
% Additionally, CLIP visual features alone did best with LSTM aggregation. T

In future work we hope to learn hierarchical representations in order to encode global information such as that of Screen2Vec as well as local information from icon embeddings. Taking advantage of the tree structure from the view hierarchy via Transformers or Graph Neural Networks may help learn structured app features. Additionally, all current approaches do not take into account any notion of app `affordance,' \ie, which UI elements are most actionable.

